Iterated Energy-based Flow Matching for Sampling from Boltzmann Densities

In this work, we consider the problem of training a generator from evaluations of energy functions or unnormalized densities. This is a fundamental problem in probabilistic inference, which is crucial for scientific applications such as learning the 3D coordinate distribution of a molecule. To solve this problem, we propose iterated energy-based flow matching (iEFM), the first off-policy approach to train continuous normalizing flow (CNF) models from unnormalized densities. We introduce the simulation-free energy-based flow matching objective, which trains the model to predict the Monte Carlo estimation of the marginal vector field constructed from known energy functions. Our framework is general and can be extended to variance-exploding (VE) and optimal transport (OT) conditional probability paths. We evaluate iEFM on a two-dimensional Gaussian mixture model (GMM) and an eight-dimensional four-particle double-well potential (DW-4) energy function. Our results demonstrate that iEFM outperforms existing methods, showcasing its potential for efficient and scalable probabilistic modeling in complex high-dimensional systems.

==> sections/background.tex <==
\section{Preliminaries}
We are interested in sampling from the Boltzmann distribution $\mu: \mathbb{R}^d \rightarrow \mathbb{R}$ of an energy function $\mathcal{E}: \mathbb{R}^d \rightarrow \mathbb{R}$, defined as:
\begin{equation*}
     \mu(x) = \frac{\exp(-\mathcal{E}(x))}{Z}, Z = \int_{\mathbb{R}^d} \exp(-\mathcal{E}(x))dx.
\end{equation*}
The normalizing constant $Z$ is unknown, making direct evaluation of $\mu$ infeasible. Additionally, we assume no available sample from $\mu$, although we can compute the unnormalized density via the energy function $\mathcal{E}$. 

To solve this problem, we need a novel energy-based training algorithm that relies solely on energy function to train probabilistic model. This section outlines the recent SOTA energy-based training method for denoising diffusion model and flow matching objective for CNF model.

%\subsection{Iterated Denoising Energy Matching}
%Iterated Denoising Energy Matching (iDEM) is an energy-based training algorithm designed for denoising diffusion models to sample from a Boltzmann distribution. The iDEM algorithm comprises two main components: an inner loop that optimizes the DEM objective, and an outer loop that explores the sample point for which DEM objective is optimized.

%The DEM objective involves regressing the score network to the estimated score of the noised distribution at a given point and time, functioning as an off-policy objective. iDEM employs a replay buffer to determine the points at which regression is performed. Following the fitting of the DEM objective in the inner loop, samples are generated by integrating a stochastic differential equation (SDE) using the score network, and these samples are subsequently added to the replay buffer. This iterative process is repeated until training converges.

%It is important to note that any probabilistic model $p_\theta$ can adopt the iDEM exploration strategy by sampling from $p_\theta$ instead of using SDE integration. However, for tractable training, the inner loop fitting objective for $p_\theta$ must be efficiently evaluated (e.g., the simulation-free DEM objective for diffusion models). This highlights the need for simulation-free off-policy objectives to extend iDEM to allow the training of Continuous Normalizing Flow (CNF) models.

\subsection{Flow Matching}
\label{sec:CNF and FM}
We consider a random process $\{x_t\}_{t=0}^1$ and its marginal density $p_t$ with $t \in [0,1]$ which starts at simple Gaussian prior $p_0 = N(0, \sigma_0^2)$ and ends at the target distribution $p_1 = \mu_{target}$. Let $v_t: \mathbb{R}^d \rightarrow \mathbb{R}^d$ with $t \in [0,1]$ be the time-dependent vector fields that generates $p_t$ and $u_t(-;\theta)$ be the time-dependent vector fields modeled by neural network. 

Then, the Flow Matching (FM) objective \cite{lipman2022flow} is defined as follows:
\begin{equation}
    \mathcal{L}_{\text{FM}}(\theta) = \mathbb{E}_{x, t}[\lVert u_t(x; \theta) - v_t(x) \rVert_2^2].
\end{equation} 
For fixed marginal probability density path $p_t$, there can be many possible $v_t$ generating $p_t$. One of the natural choice is
\begin{equation}
    \label{eqn:vt_as_integral}
    v_t(x) = \int {v_t(x|x_1)}\frac{p_t(x|x_1)p_1(x_1)}{p_t(x)}dx_1,
\end{equation}
where $v_t(x|x_1)$ is a vector field that generates conditional probability path $p_t(x|x_1)$. Here, $v_t$ is called marginal vector field (MVF) since it generates marginal probability paths $p_t$.

%However, the integral in \cref{eqn:vt_as_integral} is intractable in generative modeling since the number of sample from $p_1$ is limited by the size of the datasets. To bypass such limitation, conditional flow matching (CFM) is proposed. 
%\todo{Is it correct...? Why not using training set to estimate MVFs?}
%\todo{Why conditional flow matching cannot be adapt iDEM exploration strategy...?}

After trained by optimizing FM or equivalent CFM objective, we can generate sample by solving ODE with initial value $x_0$ from prior $p_0$.
\begin{equation*}
    \frac{dx}{dt} = u_t(x;\theta) \text{ where } x(0) = x_0
\end{equation*}
